A ribbon ZX calculus for gauge theory

ZX calculus provides a graphical formalism for reasoning about quantum processes, built from two interacting Frobenius algebras associated with the Z and X bases of a qubit. While it has found widespread application in quantum information and computing, its relationship to quantum field theory has only recently begun to be explored. In this work, we further develop this connection by providing a generalization of ZX calculus to two-dimensional Yang Mills theory with a compact gauge group. The key observation is that both frameworks can be organized around the Hopf Frobenius algebraic structure associated with a group algebra, which can in turn be described by the diagrammatics of two dimensional topological quantum field theory. Given the well known relationship between gauge theory and gravity in two and three dimensions, our work paves the way for applications of ZX to low dimensional gravity.

==> notes/Hadamard.tex <==
\paragraph{Hadamard}
To go from the Z to the X spider, we would like to rotate the ribbon by 90 degrees. 
\begin{align}
\includegraphics[scale=.1]{figures/hadamard.png}
\end{align}
Intuitively, this rotaion by 90 relates the fusion and stacking process described by the Z and X spiders. However, technically, such a rotation can not be made precise in general:  The representations basis is discrete, whereas the group basis is continuous, and there is no one to one map between them.   It is only in the special case of $L^{2}(R)$ or $L^{2}(\mathbb{Z}^d)$, that this is possible because of Pontryagin self duality.
